MoGenTS: Motion Generation based on Spatial-Temporal Joint Modeling

Motion generation from discrete quantization offers many advantages over continuous regression, but at the cost of inevitable approximation errors. Previous methods usually quantize the entire body pose into one code, which not only faces the difficulty in encoding all joints within one vector but also loses the spatial relationship between different joints. Differently, in this work we quantize each individual joint into one vector, which i) simplifies the quantization process as the complexity associated with a single joint is markedly lower than that of the entire pose; ii) maintains a spatial-temporal structure that preserves both the spatial relationships among joints and the temporal movement patterns; iii) yields a 2D token map, which enables the application of various 2D operations widely used in 2D images. Grounded in the 2D motion quantization, we build a spatial-temporal modeling framework, where 2D joint VQVAE, temporal-spatial 2D masking technique, and spatial-temporal 2D attention are proposed to take advantage of spatial-temporal signals among the 2D tokens. Extensive experiments demonstrate that our method significantly outperforms previous methods across different datasets, with a 26.6% decrease of FID on HumanML3D and a 29.9% decrease on KIT-ML. Project page: https://aigc3d.github.io/mogents.

==> sections/3_method.tex <==

\section{Method}
\vspace{-2mm}
\subsection{Problem Statement}
\vspace{-2mm}

\textbf{Motion Quantization.}
Given a motion sequence $\{\mathbf{M}_t\}_{t=1}^{T}$, the objective is to construct an optimal codebook $\mathbf{C}=\{\mathbf{c}_i\}_{i=1}^{C}$ capable of accurately representing this sequence, so that the encoded motion features $\mathbf{V}$ could be substituted by the corresponding codes $c_i$ from the codebook with the minimum loss, resulting in a discrete token sequence $\{\mathbb{O}\}$, representing the input motion.

\textbf{Motion Generation.}
Given the textual prompt $\mathbf{T}$, the task of our framework is to generate the indices of the tokens $\{\mathbb{O}\}$, so that the vectors corresponding to these tokens could be decoded into a motion sequence aligned with the input text.

\vspace{-2mm}
\subsection{Overview}
\vspace{-2mm}

The overview of our method is illustrated in Figure~\ref{fig:framework}.
Our framework could be divided into two parts, motion quantization and motion generation.
In the quantization phase, we first represent the input motion sequence in the joint-time structure, and encode it into a 2D vector map.
Subsequently, the vectors are quantized into codes of a codebook, represented by the indices of the selected codebook entries, i.e., the joint tokens.
Therefore, after the quantization, the input motion sequence is converted to tokens arranged in a 2D structure, where one dimension is spatial while the other one is temporal.
This results in a 2D motion map, which is similar to a 2D image.
In the generation phase, we mask the 2D token map with a temporal-spatial 2D masking strategy, and then use a 2D transformer to predict the masked tokens, conditioned on the embedding $\mathbf{T}$ of the given text prompt.
The 2D motion transformer considers both spatial attention and temporal attention between different 2D tokens. The 2D position embedding $\mathbf{P}$ is also used to convey the spatial and temporal locations of each token.
Finally, the generated tokens are decoded back into a motion sequence that aligns with the given textual prompt, thus completing the process of text-driven motion generation.



\begin{figure}[]
% \vspace{-3mm}
\centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/vq.pdf}
\vspace{-7mm}
\caption{The structure of our spatial-temporal 2D Joint VQ-VAE for motion quantization.
}
\label{fig:vq}
\vspace{-5mm}
\end{figure}


\vspace{-2mm}
\subsection{Spatial-temporal 2D Joint Quantization of Motion}
\vspace{-2mm}
% details of 2D CNN?

Directly regressing the continuous motion sequence is not easy.
Thus, we perform motion quantization following previous methods~\cite{momask} to convert the regression problem to a classification problem, but differently, we quantize each joint rather than the whole-body pose.
Therefore, we organize the motion sequence in a 2D structure and process it as a 2D map, as illustrated in Figure~\ref{fig:vq}.
For a motion with sequence length $T$ and joint number $J$, we employ a 2D convolutional network to encode the motion joints $\mathbf{J}=\{\mathbf{j}_t^j\}_{t=1, ..., T}^{j=1, ..., J}$ into 2D vectors $\mathbf{V}=\{\mathbf{v}_t^j\}_{t=1, ..., T}^{j=1, ..., J}$, where each vector $\mathbf{v}_t^j$ corresponds to time $t$ and joint $j$, as
\begin{equation}
    \{ \mathbf{v}_t^j \} = \mathcal{E}~ ( \{ \mathbf{j}_t^j \} ),
\end{equation}
where $\mathcal{E}$ denotes the encoder network composed of two convolutional residual blocks.
Then we quantize the vector with a codebook, i.e. we replace the vector $\mathbf{v}_t^j$ with its nearest code entry $\mathbf{\tilde{v}}_t^j$ in a preset codebook $\mathbf{C}=\{\mathbf{c}_i\}_{i=1}^{C}$, as
\begin{equation}
    \{ \mathbf{\tilde{v}}_t^j \} = \mathcal{Q}~ ( \{ \mathbf{v}_t^j \} ), ~~~
    \mathcal{Q}: \mathbf{\tilde{v}}_t^j = \mathbf{c}_i ~\text{where}~ i = \argmin_i || \mathbf{c}_i - \mathbf{v}_t^j ||_2.
\end{equation}
Here $\mathcal{Q}$ denotes the quantization process.
After the quantization, the decoder $\mathcal{D}$ decodes the approximate vectors $\mathbf{\tilde{v}}_t^j$ to get the original joint information, as
\begin{equation}
    \{ \mathbf{\tilde{j}}_t^j \} = \mathcal{D}~ ( \{ \mathbf{\tilde{v}}_t^j \} )
    = \mathcal{D}~ (~ \mathcal{Q}~ (~ \mathcal{E}~ (~ \{ \mathbf{j}_t^j \} ~ ) ~ ) ~ ).
\end{equation}


Finally, the auto-encoding network is optimized by a loss considering both the vector approximation and the decoded joints, as
\begin{equation}
    \mathcal{L}_{vq} = \sum_{t,j} || \mathbf{\tilde{j}}_t^j - \mathbf{j}_t^j ||_1 + \alpha || \mathbf{\tilde{v}}_t^j - \mathbf{v}_t^j ||_2,
\end{equation}
where $\alpha$ denotes a weighting factor. We also employ the residual VQ-VAE structure, exponential moving average, and codebook reset following previous methods~\cite{T2MGPT, momask}.



\vspace{-2mm}
\subsection{Temporal-spatial 2D Token Masking}
\label{sec:mask}
\vspace{-2mm}

After quantization of the motion joints, we obtain a 2D token map $\{ \mathbb{O}_t^j \}$ as shown in Figure~\ref{fig:attn}.
We follow language models~\cite{bert,MaskGIT} to perform random masking, but differently, here our tokens are in a 2D structure and there are totally ${T} \times {J}$ tokens.
In this case, performing a 1D masking strategy ignoring the spatial-temporal relationship is not optimal, which applies the same masking strategy to all tokens.
For example, it rarely appears that all joints in one frame are masked in the meantime. Networks trained in this way cannot work well in generating new motions, since the generation requires starting from an all-masked motion.

To solve this problem, we propose a 2D temporal-spatial masking strategy.
We first perform the masking in only the temporal dimension and randomly mask the frames in the sequence. 
Once one frame is masked, all joints in this frame are masked, as illustrated in Figure~\ref{fig:attn} (a).
After the temporal masking, we perform spatial masking on the remaining unmasked frames.
Specifically, we randomly do the second masking in the spatial dimension for all joints of an unmasked frame.
All masked tokens are replaced by the $\mathbb{O}_\text{mask}$ token, which denotes that this location is masked and predicted. Note that there is an underlying graph structure among the joints and that we have tried graph-based masking strategies. However, we find that the simple random masking strategy works the best. One interpretation is that it helps encode long-range correlations of joints in human motions, c.f.~\cite{DBLP:conf/cvpr/ChiHCLHR22}.  

The temporal and spatial masking strategies adopt the same mask ratio schedule following~\cite{chang2022maskgit, muse}.
This ratio is computed as
\begin{equation}
    \gamma(\tau) = \cos(\frac{\pi \tau}{2}),
\end{equation}
where $\tau \in [0, 1]$.
In training, $\tau \sim \mathbf{U}(0, 1)$ is uniformly sampled, leading to a mask ratio $\gamma(\tau)$. Then according to this ratio, $\gamma(\tau)\times T\times J$ tokens are randomly selected to be masked in temporal masking, and $\gamma(\tau) \times J$ tokens are randomly selected to be masked for one frame in the spatial masking.
To add more disturbance to the masked prediction, the remasking mechanism in BERT~\cite{bert} is also employed: If a token $\mathbb{O}_t^j$ is selected to be masked, it would be replaced with $\mathbb{O}_\text{mask}$ with an 80\% probability, would be replaced with a random token $\mathbb{O}_{i}$ with a 10\% probability, and remains unchanged with a 10\% probability.
After the temporal-spatial masking, we obtain a masked 2D token map for subsequent networks to predict.



\begin{figure}[]
% \vspace{-3mm}
\centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/attn.pdf}
\vspace{-6mm}
\caption{The temporal-spatial masking strategy (a) and the spatial-temporal attention (b) for motion generation.
}
\label{fig:attn}
\vspace{-6mm}
\end{figure}





\subsection{Spatial-temporal 2D Motion Generation}

\subsubsection{Spatial-Temporal Motion Transformer}
\label{sec:transformer}

Given a text input and a masked token map, we use a transformer network to predict the tokens at the masked locations.
There are three attentions performed in this transformer: spatial-temporal 2D attention, spatial attention, and temporal attention, as illustrated in Figure~\ref{fig:attn}(b). 
% In the following, we first introduce their designs, including their strengths and limitations. We then describe a network design that combines their strength. 

\textbf{Spatial-Temporal 2D Attention.}
For the spatial-temporal attention, we first extract the text feature embedding using CLIP~\cite{CLIP}, resulting in a text token $\mathbb{O}_\text{text}$.
Then we add a 2D position encoding~\cite{wang2019translating} to the 2D token map.
The position encoding $\mathbf{P}_t^j$ is computed by the sinusoidal function in the spatial dimension $j$ and in the temporal dimension $t$, respectively, so it provides both the spatial position and the temporal position information for the subsequent attention network.
After the 2D position embedding, we flatten the 2D token map to the 1D structure and prepend the text embedding to the flattened token sequence.
Then we perform the 1D attention in the flattened spatial-temporal dimension, where the spatial and temporal relationship is reserved by the 2D position encoding, as
\begin{equation}
    \mathcal{A}_{s-t} = \text{SoftMax}(Q \cdot K / \sqrt{d} + \mathbf{P}) V,
\end{equation}
where $Q, K, V \in \mathbb{R}^{(JT+1)\times d}$ are the query, key, and value matrices, d is the feature dimension, and $JT+1$ is the number of tokens.
This bidimensional attention is performed in a long sequence of $JT+1$ tokens. Its strength is that it is able to learn patterns in the full spatial-temporal space. The limitation is that the mix of spatial and temporal information is too complex to learn. The resulting patterns are inaccurate. 

\textbf{Joint Spatial Attention.}
Joint spatial attention is the one-dimensional attention in only the spatial dimension.
As shown in Figure~\ref{fig:attn}(b), we ignore the temporal dimension and rearrange the 2D tokens. 
The tokens of different time frames are regarded as different batches, and then the attention is only calculated between different joints on each time batch, as
\begin{equation}
    \mathcal{A}_{s} = \text{SoftMax}(Q_s \cdot K_s / \sqrt{d} + \mathbf{P}) V_s,
\end{equation}
where $Q_s, K_s, V_s \in \mathbb{R}^{J\times d}$.
This spatial attention equally works on the joints of any time frame, so it could capture the inner relationship between different joints without the influence of temporal information.
The advantage of this attention module is that it is easier to learn. However, it only guarantees the rationality of the different joints in one pose, regardless of whether the input text is or what the target motion is.


\textbf{Joint Temporal Attention.}
Similar to spatial attention, we also perform one-dimensional attention in only the temporal dimension.
As shown in Figure~\ref{fig:attn}(b), we ignore the spatial dimension and rearrange the 2D tokens.
The tokens of different joints are regarded as different batches, and then the attention is only calculated between different times on each joint batch, as
\begin{equation}
    \mathcal{A}_{t} = \text{SoftMax}(Q_t \cdot K_t / \sqrt{d} + \mathbf{P}) V_t,
\end{equation}
where $Q_s, K_s, V_s \in \mathbb{R}^{T\times d}$.
This temporal attention works equally on the time sequence of any joint. Similar to joint spatial attention, this attention module is easier to learn. However, it mostly captures the change in motion of the joint and guarantees the rationality of the movement of one joint, such as motion smoothness.

\textbf{Integration of attention modules.} Our approach applies spatial-temporal 2D attention, joint spatial attention, and joint temporal attention in a sequential manner. Here the spatial-temporal 2D attention provides the initialization, and joint spatial attention and joint-temporal attention offer regualarization.

\subsubsection{Training and Inference.}

\textbf{Training.}
In the training, we use the spatial-temporal motion transformer to predict the probability logits of all $C$ tokens $\hat{y}_i$ in the masked positions.
Then a cross-entropy loss is computed between the prediction $\hat{y}$ and the target $y$, as
\begin{equation}
    \mathcal{L}_{\text{mask}} = - \sum_{\text{mask}}\sum_{i=1}^{C} y_i \log(\hat{y}_i)+(1-y_i)\log(1-\hat{y}_i).
\end{equation}

We also employ the residual structure following previous methods~\cite{momask}, and use a residual spatial-temporal motion transformer to improve motion accuracy.
The structure of the residual transformer is the same as that of the mask transformer, including spatial-temporal attention, spatial attention, and temporal attention.
In training, we randomly select one layer $l$ from the $L$ residual layers to learn. All tokens in the preceding layers $[0:l]$ are summed as the input of the residual transformer.
The prediction of the $l$-th layer tokens is also optimized by the cross-entropy loss.


\textbf{Inference.}
In the inference, the generation starts from an empty token map, i.e., all tokens are masked. 
The prediction of the masked tokens is repeated by $N$ iterations.
In each iteration, we build the probability distribution of $C$ tokens from the SoftMax of the predicted logits, and sample the output from the distribution.
In the next iteration, according to the schedule shown in Section~\ref{sec:mask} with $\tau=n/N$, low-score tokens are selected to be masked and predicted again, until $n$ reaches $N$.
Once the iterative masked generation is finished, the residual transformer progressively predicts the residual tokens of the residual VQ layers.
Afterward, the base tokens plus the residual tokens are decoded by the VQVAE decoder to get the final generated motion.

==> sections/4_experiments.tex <==

\setlength{\tabcolsep}{4.5pt}
\begin{table}[]
% \vspace{-2mm}
\small
\centering
% \scalebox{1}{
\begin{tabular}{l c c c c c c }
\toprule
Methods & FID $\downarrow$ & Top1 $\uparrow$ & Top2 $\uparrow$ & Top3 $\uparrow$  & MM-Dist $\downarrow$ & Diversity $\rightarrow$ \\ %& MultiModality
\midrule
Ground Truth & $0.002^{\pm .000}$ & $0.511^{\pm .003}$ & $0.703^{\pm .003}$ & $0.797^{\pm .002}$  & $2.974^{\pm .008}$ & $9.503^{\pm .065}$ \\ % &-
\midrule
TEMOS~\cite{temos} & $3.734^{\pm .028}$ & $0.424^{\pm .002}$ & $0.612^{\pm .002}$ & $0.722^{\pm .002}$  & $3.703^{\pm .008}$ & $8.973^{\pm .071}$ \\ %& $0.368^{\pm .018}$
TM2T~\cite{TM2T} & $1.501^{\pm .017}$ & $0.424^{\pm .003}$ & $0.618^{\pm .003}$ & $0.729^{\pm .002}$  & $3.467^{\pm .011}$ & $8.589^{\pm .076}$ \\ % $2.424^{\pm .093}$ \\
T2M~\cite{t2m} & $1.087^{\pm .021}$ & $0.455^{\pm .003}$ & $0.636^{\pm .003}$ & $0.736^{\pm .002}$  & $3.347^{\pm .008}$ & $9.175^{\pm .083}$ \\ %& $2.219^{\pm .074}$ \\
MDM~\cite{MDM} & $0.544^{\pm .044}$ & - & - & $0.611^{\pm .007}$  & $5.566^{\pm .027}$ & $9.559^{\pm .086}$ \\ % & $2.799^{\pm .072}$ \\
MLD~\cite{MLD} & $0.473^{\pm .013}$ & $0.481^{\pm .003}$ & $0.673^{\pm .003}$ & $0.772^{\pm .002}$  & $3.196^{\pm .010}$ & $9.724^{\pm .082}$ \\ % & $2.413^{\pm .079}$ \\
MotionDiffuse~\cite{MotionDiffuse} & $0.630^{\pm .001}$ & $0.491^{\pm .001}$ & $0.681^{\pm .001}$ & $0.782^{\pm .001}$  & $3.113^{\pm .001}$ & $9.410^{\pm .049}$ \\ %& $1.553^{\pm .042}$ \\
PhysDiff~\cite{PhysDiff} & $0.433$ & - & - & $0.631$  & - & - \\
MotionGPT~\cite{motiongpt} & $0.567$ & - & - & -  & $3.775$ & $9.006$ \\
T2M-GPT~\cite{T2MGPT} & $0.141^{\pm .005}$ & $0.492^{\pm .003}$ & $0.679^{\pm .002}$ & $0.775^{\pm .002}$  & $3.121^{\pm .009}$ & $9.761^{\pm .081}$ \\ % $1.831^{\pm .048}$ \\
M2DM~\cite{M2DM} & $0.352^{\pm .005}$ & $0.497^{\pm .003}$ & $0.682^{\pm .002}$ & $0.763^{\pm .003}$  & $3.134^{\pm .010}$ & $9.926^{\pm .073}$ \\ % & $3.587^{\pm .072}$ \\
Fg-T2M~\cite{FgT2M} & $0.243^{\pm .019}$ & $0.492^{\pm .002}$ & $0.683^{\pm .003}$ & $0.783^{\pm .002}$  & $3.109^{\pm .007}$ & $9.278^{\pm .072}$ \\ % & $1.614^{\pm .049}$ \\
%& $1.869^{\pm .089}$ \\
% ReMoDiffuse~\cite{remodiffuse} & $0.510^{\pm .005}$ & $0.698^{\pm .006}$ & $0.795^{\pm .004}$ & $0.103^{\pm .004}$ & $2.974^{\pm .016}$ & $9.018^{\pm .075}$ \\ % $1.795^{\pm .043}$ \\
AttT2M~\cite{AttT2M} & $0.112^{\pm .006}$ & $0.499^{\pm .003}$ & $0.690^{\pm .002}$ & $0.786^{\pm .002}$  & $3.038^{\pm .007}$ & $9.700^{\pm .090}$ \\ %& $2.452^{\pm .051}$ \\
DiverseMotion~\cite{DiverseMotion} & $0.072^{\pm .004}$ & $0.515^{\pm .003}$ & $0.706^{\pm .002}$ & $0.802^{\pm .002}$  & $2.941^{\pm .007}$ & $9.683^{\pm .102}$ \\ 
ParCo~\cite{ParCo} & $0.109^{\pm .005}$ & $0.515^{\pm .003}$ & $0.706^{\pm .003}$ & $0.801^{\pm .002}$  & $2.927^{\pm .008}$ & $9.576^{\pm .088}$ \\ %& $1.382^{\pm .060}$ \\
MMM~\cite{MMM} & $0.080^{\pm .003}$ & $0.504^{\pm .003}$ & $0.696^{\pm .003}$ & $0.794^{\pm .002}$  & $2.998^{\pm .007}$ & $9.411^{\pm .058}$ \\ % & $1.164^{\pm .041}$ \\
MoMask~\cite{momask} & $0.045^{\pm .002}$ & $0.521^{\pm .002}$ & $0.713^{\pm .002}$ & $0.807^{\pm .002}$  & $2.958^{\pm .008}$ & - \\ % & $1.241^{\pm .040}$ \\
% MoMask*~\cite{momask} & $0.078^{\pm .004}$ & $0.510^{\pm .003}$ & $0.704^{\pm .003}$ & $0.802^{\pm .002}$  & $3.014^{\pm .008}$ & $9.544^{\pm .090}$ \\ % & $1.302^{\pm .041}$ \\
Ours & $\mathbf{0.033}^{\pm .001}$ & $\mathbf{0.529}^{\pm .003}$ & $\mathbf{0.719}^{\pm .002}$ & $\mathbf{0.812}^{\pm .002}$  & $\mathbf{2.867}^{\pm .006}$ & $9.570^{\pm .077}$  \\ %& $0.793^{\pm .025}$ \\
\midrule
\midrule
Ground Truth & $0.031^{\pm .004}$ & $0.424^{\pm .005}$ & $0.649^{\pm .006}$ & $0.779^{\pm .006}$  & $2.788^{\pm .012}$ & $11.080^{\pm .097}$ \\ % & - \\
\midrule
TEMOS~\cite{temos} & $3.717^{\pm .028}$ & $0.353^{\pm .002}$ & $0.561^{\pm .002}$ & $0.687^{\pm .002}$  & $3.417^{\pm .008}$ & $10.84^{\pm .100}$ \\ % & $0.532^{\pm .018}$ \\
TM2T~\cite{TM2T} & $3.599^{\pm .153}$ & $0.280^{\pm .005}$ & $0.463^{\pm .006}$ & $0.587^{\pm .005}$  & $4.591^{\pm .026}$ & $9.473^{\pm .117}$ \\ % & $3.292^{\pm .081}$ \\
T2M~\cite{t2m} & $3.022^{\pm .107}$ & $0.361^{\pm .005}$ & $0.559^{\pm .007}$ & $0.681^{\pm .007}$  & $3.488^{\pm .028}$ & $10.72^{\pm .145}$ \\ % & $2.052^{\pm .107}$ \\
MDM~\cite{MDM} & $0.497^{\pm .021}$ & - & - & $0.396^{\pm .004}$  & $9.191^{\pm .022}$ & $10.85^{\pm .109}$ \\ % & $1.907^{\pm .214}$ \\
MLD~\cite{MLD} & $0.404^{\pm .027}$ & $0.390^{\pm .008}$ & $0.609^{\pm .008}$ & $0.734^{\pm .007}$  & $3.204^{\pm .027}$ & $10.80^{\pm .117}$ \\ % & $2.192^{\pm .071}$ \\
MotionDiffuse~\cite{MotionDiffuse} & $1.954^{\pm .062}$ & $0.417^{\pm .004}$ & $0.621^{\pm .004}$ & $0.739^{\pm .004}$  & $2.958^{\pm .005}$ & $11.10^{\pm .143}$ \\ % & $0.730^{\pm .013}$ \\
MotionGPT~\cite{motiongpt} & $0.597$ & - & - & -  & $3.394$ & $10.54$ \\
T2M-GPT~\cite{T2MGPT} & $0.514^{\pm .029}$ & $0.416^{\pm .006}$ & $0.627^{\pm .006}$ & $0.745^{\pm .006}$  & $3.007^{\pm .023}$ & $10.86^{\pm .094}$ \\ % & $1.570^{\pm .039}$ \\
M2DM~\cite{M2DM} & $0.515^{\pm .029}$ & $0.416^{\pm .004}$ & $0.628^{\pm .004}$ & $0.743^{\pm .004}$  & $3.015^{\pm .017}$ & $11.417^{\pm .097}$ \\ % & $3.325^{\pm .037}$ \\
Fg-T2M~\cite{FgT2M} & $0.571^{\pm .047}$ & $0.418^{\pm .005}$ & $0.626^{\pm .004}$ & $0.745^{\pm .004}$  & $3.114^{\pm .015}$ & $10.93^{\pm .083}$ \\ % & $1.019^{\pm .029}$ \\
% & $2.062^{\pm .079}$ \\
% ReMoDiffuse~\cite{remodiffuse} & $0.427^{\pm .014}$ & $0.641^{\pm .004}$ & $0.765^{\pm .055}$ & $0.155^{\pm .006}$ & $2.814^{\pm .012}$ & $10.80^{\pm .105}$ \\ % & $1.239^{\pm .028}$ \\
AttT2M~\cite{AttT2M} & $0.870^{\pm .039}$  & $0.413^{\pm .006}$ & $0.632^{\pm .006}$ & $0.751^{\pm .006}$ & $3.039^{\pm .021}$ & $10.96^{\pm .123}$ \\ % & $2.281^{\pm .047}$ \\
DiverseMotion~\cite{DiverseMotion} & $0.468^{\pm .098}$ & $0.416^{\pm .005}$ & $0.637^{\pm .008}$ & $0.760^{\pm .011}$  & $2.892^{\pm .041}$ & $10.873^{\pm .101}$ \\ 
ParCo~\cite{ParCo} & $0.453^{\pm .027}$  & $0.430^{\pm .004}$ & $0.649^{\pm .007}$ & $0.772^{\pm .006}$  & $2.820^{\pm .028}$ & $10.95^{\pm .094}$ \\ % & $1.245^{\pm .022}$ \\
MMM~\cite{MMM} & $0.429^{\pm .019}$ & $0.381^{\pm .005}$ & $0.590^{\pm .006}$ & $0.718^{\pm .005}$  & $3.146^{\pm .019}$ & $10.633^{\pm .097}$ \\ % & $1.105^{\pm .026}$ \\
MoMask~\cite{momask} & $0.204^{\pm .011}$ & $0.433^{\pm .007}$ & $0.656^{\pm .005}$ & $0.781^{\pm .005}$  & $2.779^{\pm .022}$ & - \\ % & $1.131^{\pm .043}$ \\
Ours & $\mathbf{0.143}^{\pm .004}$ & $\mathbf{0.445}^{\pm .006}$ & $\mathbf{0.671}^{\pm .006}$ & $\mathbf{0.797}^{\pm .005}$  & $\mathbf{2.711}^{\pm .024}$ & ${10.918}^{\pm .090}$ \\ % & $0.839^{\pm .035}$ \\
\bottomrule
\end{tabular}
% }
% \vspace{-3mm}
\caption{Evaluation on the HumanML3D dataset (upper half) and the KIT-ML dataset (lower half).
}
\label{tab:eval_humanml}
\vspace{-5mm}
\end{table}
\setlength{\tabcolsep}{6pt}



% \begin{table*}[]
% % \vspace{-2mm}
% \small
% \centering
% \begin{tabular}{l c c c c c c}
% \toprule
% Methods & FID $\downarrow$ & Top1 $\uparrow$ & Top2 $\uparrow$ & Top3 $\uparrow$  & MultiModal Dist $\downarrow$ & Diversity $\rightarrow$ \\ %MultiModality  \\
% \midrule
% GT & $0.031^{\pm .004}$ & $0.424^{\pm .005}$ & $0.649^{\pm .006}$ & $0.779^{\pm .006}$  & $2.788^{\pm .012}$ & $11.080^{\pm .097}$ \\ % & - \\
% \midrule
% TEMOS~\cite{temos} & $3.717^{\pm .028}$ & $0.353^{\pm .002}$ & $0.561^{\pm .002}$ & $0.687^{\pm .002}$  & $3.417^{\pm .008}$ & $10.84^{\pm .100}$ \\ % & $0.532^{\pm .018}$ \\
% TM2T~\cite{TM2T} & $3.599^{\pm .153}$ & $0.280^{\pm .005}$ & $0.463^{\pm .006}$ & $0.587^{\pm .005}$  & $4.591^{\pm .026}$ & $9.473^{\pm .117}$ \\ % & $3.292^{\pm .081}$ \\
% T2M~\cite{t2m} & $3.022^{\pm .107}$ & $0.361^{\pm .005}$ & $0.559^{\pm .007}$ & $0.681^{\pm .007}$  & $3.488^{\pm .028}$ & $10.72^{\pm .145}$ \\ % & $2.052^{\pm .107}$ \\
% MDM~\cite{MDM} & $0.497^{\pm .021}$ & - & - & $0.396^{\pm .004}$  & $9.191^{\pm .022}$ & $10.85^{\pm .109}$ \\ % & $1.907^{\pm .214}$ \\
% MLD~\cite{MLD} & $0.404^{\pm .027}$ & $0.390^{\pm .008}$ & $0.609^{\pm .008}$ & $0.734^{\pm .007}$  & $3.204^{\pm .027}$ & $10.80^{\pm .117}$ \\ % & $2.192^{\pm .071}$ \\
% MotionDiffuse~\cite{MotionDiffuse} & $1.954^{\pm .062}$ & $0.417^{\pm .004}$ & $0.621^{\pm .004}$ & $0.739^{\pm .004}$  & $2.958^{\pm .005}$ & $11.10^{\pm .143}$ \\ % & $0.730^{\pm .013}$ \\
% MotionGPT~\cite{motiongpt} & $0.597$ & - & - & -  & $3.394$ & $10.54$ \\
% T2M-GPT~\cite{T2MGPT} & $0.514^{\pm .029}$ & $0.416^{\pm .006}$ & $0.627^{\pm .006}$ & $0.745^{\pm .006}$  & $3.007^{\pm .023}$ & $10.86^{\pm .094}$ \\ % & $1.570^{\pm .039}$ \\
% M2DM~\cite{M2DM} & $0.515^{\pm .029}$ & $0.416^{\pm .004}$ & $0.628^{\pm .004}$ & $0.743^{\pm .004}$  & $3.015^{\pm .017}$ & $11.417^{\pm .097}$ \\ % & $3.325^{\pm .037}$ \\
% Fg-T2M~\cite{FgT2M} & $0.571^{\pm .047}$ & $0.418^{\pm .005}$ & $0.626^{\pm .004}$ & $0.745^{\pm .004}$  & $3.114^{\pm .015}$ & $10.93^{\pm .083}$ \\ % & $1.019^{\pm .029}$ \\
% % & $2.062^{\pm .079}$ \\
% % ReMoDiffuse~\cite{remodiffuse} & $0.427^{\pm .014}$ & $0.641^{\pm .004}$ & $0.765^{\pm .055}$ & $0.155^{\pm .006}$ & $2.814^{\pm .012}$ & $10.80^{\pm .105}$ \\ % & $1.239^{\pm .028}$ \\
% AttT2M~\cite{AttT2M} & $0.870^{\pm .039}$  & $0.413^{\pm .006}$ & $0.632^{\pm .006}$ & $0.751^{\pm .006}$ & $3.039^{\pm .021}$ & $10.96^{\pm .123}$ \\ % & $2.281^{\pm .047}$ \\
% DiverseMotion~\cite{DiverseMotion} & $0.468^{\pm .098}$ & $0.416^{\pm .005}$ & $0.637^{\pm .008}$ & $0.760^{\pm .011}$  & $2.892^{\pm .041}$ & $10.873^{\pm .101}$ \\ 
% ParCo~\cite{ParCo} & $0.453^{\pm .027}$  & $0.430^{\pm .004}$ & $0.649^{\pm .007}$ & $0.772^{\pm .006}$  & $2.820^{\pm .028}$ & $10.95^{\pm .094}$ \\ % & $1.245^{\pm .022}$ \\
% MMM~\cite{MMM} & $0.429^{\pm .019}$ & $0.381^{\pm .005}$ & $0.590^{\pm .006}$ & $0.718^{\pm .005}$  & $3.146^{\pm .019}$ & $10.633^{\pm .097}$ \\ % & $1.105^{\pm .026}$ \\
% MoMask~\cite{momask} & $0.204^{\pm .011}$ & $0.433^{\pm .007}$ & $0.656^{\pm .005}$ & $0.781^{\pm .005}$  & $2.779^{\pm .022}$ & - \\ % & $1.131^{\pm .043}$ \\
% Ours & $0.151^{\pm .006}$ & $0.450^{\pm .007}$ & $0.674^{\pm .008}$ & $0.797^{\pm .005}$  & $2.722^{\pm .014}$ &  \\ % & $0.839^{\pm .035}$ \\

% \bottomrule
% \end{tabular}
% % \vspace{-3mm}
% \caption{Evaluation on the KIT-ML dataset.
% }
% \label{tab:eval_kit}
% % \vspace{-2mm}
% \end{table*}



\begin{figure}[]
\centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/viz1.pdf}
  \vspace{-5mm}
\caption{Qualitative results on the test set of HumanML3D. The color from light blue to dark blue indicates the motion sequence order. An arrow indicates this sequence is unfolded in the time axis.
}
\vspace{-5mm}
\label{fig:viz1}
\end{figure}



\section{Experiments}




\vspace{-2mm}
\subsection{Datasets}
\vspace{-2mm}


We evaluate our text-to-motion model on HumanML3D~\cite{t2m} and KIT-ML~\cite{KIT} datasets.
HumanML3D consists of 14616 motion sequences and 44970 text descriptions, and KIT-ML consists of 3911 motions and 6278 texts.
Following previous methods~\cite{t2m}, 23384/1460/4383 samples are used for train/validation/test in HumanML3D, and 4888/300/830 are used for train/validation/test in KIT-ML.
The motion pose is extracted into the motion feature with dimensions of 263 and 251 for HumanML3D and KIT-ML respectively.
The motion feature contains global information including the root velocity, root height, and foot contact, and local information including local joint position, velocity, and rotations in root space.
The local joint information corresponds to 22 and 21 joints of SMPL~\cite{SMPL} for HumanML3D and KIT-ML respectively.


\vspace{-2mm}
\subsection{Implementation details}
\vspace{-2mm}

Our framework is trained on an NVIDIA A100 GPU with PyTorch.
The batch size is set to 256 and the learning rate is set to 2e-4.
To quantize the motion data into our 2D structure, we restructure the pose in the datasets to a joint-based format, with the size of $12 \times J$.
The data is then represented by the joint VQ codebook comprised of 256 codes, each with a dimension of 1024.
Due to the global information included in the HumanML3D data representation, we also incorporate an additional global VQ codebook of the same size to encode the global information.
For the residual structure, the number of residual layers is set to 5 following previous methods~\cite{momask}.
Both the encoder and decoder are constructed from 2 convolutional residual blocks with a downscale of 4.
The transformers in our model are all set to have 6 layers, 6 heads, and 384 latent dimensions.
The parameter $\alpha$ is set to 1 and $N$ is set to 10.
More details are described in the supplementary material.



\setlength{\tabcolsep}{3pt}
\begin{wraptable}{r}{0.65\textwidth}
\vspace{-12mm}
% \vspace{-2mm}
\small
\centering
\begin{tabular}{l c c c c }
\toprule
\multirow{2}*{Methods} & \multicolumn{2}{c}{HumanML3D} & \multicolumn{2}{c}{KIT-ML} \\
\cmidrule{2-5}
 & FID $\downarrow$ & MPJPE $\downarrow$ & FID $\downarrow$ & MPJPE $\downarrow$ \\
\midrule
TM2T~\cite{TM2T} & $0.307$ & $230.1$ & - & - \\ 
M2DM~\cite{M2DM} & $0.063$ & - & $0.413$ & - \\ 
T2M-GPT~\cite{T2MGPT} & $0.070$ & $58.0$ & $0.472$ & -  \\ 
MoMask~\cite{momask} & $0.019^{\pm .000}$ & $29.5^{\pm .0}$ & $0.112^{\pm .002}$ & $37.2^{\pm .1}$  \\ 
Ours & $\mathbf{0.005}^{\pm .000}$ & $\mathbf{13.8}^{\pm .0}$ & $\mathbf{0.019}^{\pm .001}$ & $\mathbf{17.4}^{\pm .1}$ \\
\bottomrule
\end{tabular}
% \vspace{-3mm}
\caption{Evaluation of motion quantization on HumanML3D dataset and KIT-ML dataset. MPJPE is measured in millimeters.
}
\label{tab:eval_vqvae}
\vspace{-3mm}
\end{wraptable}
\setlength{\tabcolsep}{6pt}


\subsection{Evaluation}

We evaluate both motion quantization and motion generation in our framework.
The evaluation protocol strictly adheres to the standards established by previous methods~\cite{t2m,T2MGPT,momask,MMM}, using the same evaluator and metric calculation.
Each experiment is repeated 20 times and the results are reported alongside a $95\%$ statistical confidence interval.

\textbf{Evaluation of Motion Quantization.}
The core idea of our framework starts from the spatial-temporal 2D joint quantization.
Therefore, we first evaluate our VQVAE against that of previous quantization-based methods.
For a fair comparison, we temporarily configure our codebook to the same size as the previous methods~\cite{momask}, i.e., $512\times512$.
As reported in Table~\ref{tab:eval_vqvae}, the FID and MPJPE accuracy of our method exceeds previous methods by a large margin, in both the HumanML3D and the KIT-ML datasets.
This reveals that the difficulty of quantizing an individual joint is much smaller than quantizing a whole-body pose.



\textbf{Evaluation of Motion Generation.}
We then compare our model to previous text-to-motion works, including both the continuous regression-based methods and the discrete quantization-based methods.
From the results reported in Table~\ref{tab:eval_humanml}, our method outperforms all previous methods on both the HumanML3D and the KIT-ML datasets, which demonstrates the effectiveness of our method.
Specifically, the FID is decreased by $26.6\%$ on HumanML3D and is decreased by $29.9\%$ on KIT-ML.
In addition, the R-precision even significantly surpasses the ground truth.
From the qualitative results displayed in Figure~\ref{fig:viz1}, we also see that our method generates motions that are better matched with the input texts compared to previous methods.





\begin{wraptable}{r}{0.5\textwidth}
% \begin{table}[]
\vspace{-8mm}
\small
\centering
\begin{tabular}{l c c }
\toprule
% Methods & \multicolumn{2}{c}{HumanML3D} & \multicolumn{2}{c}{KIT-ML} \\
 & FID $\downarrow$ & Top1 $\uparrow$  \\
\midrule
Baseline  & $0.108$     & $0.501$        \\
+ 2D VQ  & $0.194$     & $0.493$   \\
+ 2D Masking  & $0.054$     & $0.516$      \\
+ 2D Position Encoding  & $0.047$     & $0.521$    \\
+ S\&T Attn  & $0.033$     & $0.529$    \\
\bottomrule
\end{tabular}
% \vspace{-3mm}
\caption{Ablation study on HumanML3D dataset.}
\label{tab:ablation}
\vspace{-3mm}
\end{wraptable}





\subsection{Ablation Study}

\textbf{Joint 2D VQ.}
To verify the efficacy of the proposed framework, we first establish a baseline model incorporating a 1D motion VQVAE and a 1D token prediction transformer.
Then we change the VQVAE to our 2D joint VQVAE, examining its impact on both motion auto-encoding and motion generation capabilities.
According to the outcomes presented in Table~\ref{tab:eval_vqvae}, we observed a substantial enhancement in auto-encoding performance.
However, as indicated in Table~\ref{tab:ablation}, the motion generation performance deteriorates.
This decline can be attributed to the considerable increase in the number of tokens, which renders the 1D masking strategy and 1D transformer no longer adequate.


\textbf{2D Masking.}
We then change the 1D masking to temporal-spatial 2D token masking, which leads to a significant performance improvement, as depicted in Table~\ref{tab:ablation}.
This demonstrates the necessity of our 2D masking strategy, as discussed in Section~\ref{sec:mask}.


\textbf{2D Position Encoding.}
With the 2D VQ, the attention is calculated between 2D tokens, but it is not a full version of the 2D attention.
We upgrade this to spatial-temporal 2D attention by integrating the 2D position encoding, which provides both the spatial location and temporal location information.
The performance improvement brought by this encoding is recorded in Table~\ref{tab:ablation}.



\textbf{Joint Spatial and Temporal Attention.}
As discussed in Section~\ref{sec:transformer}, the mix of spatial and temporal information is complex for the bidimensional attention performed on a long sequence.
Here we inspect the benefits brought by the individual joint spatial and temporal attention mechanism.
From the results in Table~\ref{tab:ablation}, this design further improves the performance of our framework. 
% \yisheng{Yisheng: Further ablation on S\&T attention, e.g. S-T attention, S-T+J-S Attention, S-T+J-S+J-T attention?}






\begin{figure}[]
\centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/viz2.pdf}
\vspace{-7mm}
\caption{Motion Editing. The edited regions are indicated in green.
}
\label{fig:editing}
\vspace{-5mm}
\end{figure}




\subsection{Motion Editing / Inpainting}

Due to generative mask modeling, our method is capable of not only generating motions from texts, but also editing a motion by masking the tokens of any locations in both the temporal and spatial dimensions.
As shown in Figure~\ref{fig:editing}, we first mask out the motion in the temporal dimension and then generate the motions corresponding to the masked locations according to a different text prompt, resulting in a motion in which only the masked frames are edited.
Subsequently, we perform similar editing in the spatial dimension, which results in a motion where only the masked joints of masked frames are edited.
This editing mechanism could also be applied to inpainting a motion sequence or connecting two motion sequences by generating missing motions.

==> sections/5_conclusion.tex <==

\vspace{-2mm}
\section{Conclusion}
\vspace{-2mm}

This paper proposes to quantize each individual joint to one vector, generating a spatial-temporal 2D token mask for motion quantization, which reduces the approximation error in quantization, reserves the spatial information between different joints for subsequent processing, and enables the 2D operators widely used in 2D images.
Then the temporal-spatial 2D masking and spatial-temporal 2D attention are proposed to leverage the spatial-temporal information between joints for motion generation.
Extensive experiments demonstrate the efficacy of the proposed method.


\textbf{Limitations and future work.} 
Despite the improvement in the quantization, there is still the approximation error.
A large dataset for pretraining an accurate quantizer is needed in future work.

==> sections/7_checklist.tex <==


\clearpage
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction sections already reflect the paper's contributions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations have been discussed in the conclusion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have tried to include all the details and referenced work for reproduction. We will also release the code of our method.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is not included for now. But we will release the code to the public soon.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These details are described in the experiment section and appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The error bars are reported in the experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is described in the experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work conform with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no societal impact of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The used assets are properly cited in the experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
